Superconductivity in $\textit{a}$-MoGe thin films: effect of phase fluctuations with decreasing thickness and study of vortex dynamics in presence of low-frequency ac excitation

In this thesis, we have studied the evolution of superconductivity in amorphous Molybdenum Germanium ($\textit{a}$-MoGe) thin films. The work can be broken down into two parts. In the first part, we investigate the effect of decreasing thickness on the suppression of superconductivity in $\textit{a}$-MoGe thin films. Thick $\textit{a}$-MoGe thin film is a typical type-II superconductor and follows the conventional Bardeen-Cooper-Schrieffer (BCS) equation. Conventionally, it is believed that decreasing thickness will decrease the effective attractive pairing interaction because of the gradual loss of screening which holds true for large thicknesses in $\textit{a}$-MoGe. But for lower thicknesses, a new mechanism comes into the picture where superfluid density is suppressed making the superconductor vulnerable to phase fluctuations. This is known as the Bosonic mechanism, where superconductivity is destroyed due to the loss of phase coherence of the superconducting state even though the attractive pairing amplitude remains finite above the transition temperature. In the second part, we explore the electromagnetic response of vortices in $\textit{a}$-MoGe thin film by low-frequency two-coil mutual inductance technique. Penetration depth measured from the two-coil technique was earlier used to determine superfluid density. However in the present work, by analyzing the in-field penetration depth data with the help of a mean-field model proposed by Coffey and Clem, we have demonstrated a procedure of extraction of vortex parameters such as pinning restoring force constant or Labusch parameter, vortex lattice drag coefficient and pinning potential barrier for the thermally activated motion of vortices. The temperature variation of vortex parameters suggests the dominant effect of thermal fluctuations.

==> FrontMatters/declaration.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
	{\LARGE \bf DECLARATION}
\end{center}

\vskip 1cm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent This thesis is a presentation of my original research work. Wherever contributions of others are involved, 
every effort is made to indicate this clearly, with due reference to the literature, and acknowledgment of 
collaborative research and discussions.\\

\noindent The work was done under the guidance of Prof. Pratap Raychaudhuri, at the Tata Institute of Fundamental Research, Mumbai.

\vskip 3cm

\begin{flushright}
	Soumyajit Mandal
\end{flushright}
\begin{flushright}
	{\bf [Candidate's name and signature]}
\end{flushright}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip 1.5cm

\noindent In my capacity as supervisor of the candidate's thesis, I certify that the above statements are true to the best 
of my knowledge.

\vskip 3cm

\begin{flushleft}
	Prof. Pratap Raychaudhuri
\end{flushleft}
\begin{flushleft}
	{\bf [Supervisor's name and signature]}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip 0.5cm
\noindent Date:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\thispagestyle{empty}




